Automated Factual Benchmarking for In-Car Conversational Systems using Large Language Models

In-car conversational systems bring the promise to improve the in-vehicle user experience. Modern conversational systems are based on Large Language Models (LLMs), which makes them prone to errors such as hallucinations, i.e., inaccurate, fictitious, and therefore factually incorrect information. In this paper, we present an LLM-based methodology for the automatic factual benchmarking of in-car conversational systems. We instantiate our methodology with five LLM-based methods, leveraging ensembling techniques and diverse personae to enhance agreement and minimize hallucinations. We use our methodology to evaluate CarExpert, an in-car retrieval-augmented conversational question answering system, with respect to the factual correctness to a vehicle's manual. We produced a novel dataset specifically created for the in-car domain, and tested our methodology against an expert evaluation. Our results show that the combination of GPT-4 with the Input Output Prompting achieves over 90 per cent factual correctness agreement rate with expert evaluations, other than being the most efficient approach yielding an average response time of 4.5s. Our findings suggest that LLM-based testing constitutes a viable approach for the validation of conversational systems regarding their factual correctness.

==> 2-background.tex <==
% !TEX root =  root.tex
\section{Background}\label{sec:background}

\subsection{Conversational Question Answering System}

At \company, the vehicles include an in-car conversational question answering system (CQA) that the driver can use to formulate questions in natural language regarding the vehicle functionalities. In production, CQA consists of a scripted system, which only works for predefined sentences.
CQA is organized as follows. It interacts with the car's manual to get current information, saves the dialog history and uses guard rails in real-time to ensure safe output.
An orchestrator evaluates what type of inquiry the user sent, and chooses the next subsystem accordingly, similar to a microservice architecture or mixture of experts.
The user queries can consist of ways to control certain car functions, change the navigation, or questions about the car's functionalities and specifications. 

A newer release of CQA based on LLMs is currently being developed and tested. It aims to improve the users satisfaction at handling complex request beyond the vehicles information. 
In this paper, we focus on testing the subsystem that is responsible for assisting with questions about the vehicle's functionalities and specifications. 

In this context, the ground truth information is the the vehicle’s manual, the car configuration, related press articles and frequently asked questions have been parsed, embedded and stored in a vector database.
%
Using a regular Retrieval Augmented Generation (RAG) approach the question embedding is created, and k-Nearest Neighbor approximate search is used to get the top-k results closer to the given question. In the new version of CQA, Facebook AI Similarity Search (Faiss) has been utilized for the similarity search and clustering of the vectors~\cite{douze2024faiss,johnson2019billion}.
%
At the same time, a LLM accesses different prompt templates and uses the extracted answers from the retriever to generate an output. An arbitrator/answer moderator is used to control the output.

The use of the retrieved documents for the generation of the output is a critical step and this is where inconsistencies are introduced. For this reason, in our evaluation of CQA, factual consistency will serve as the most relevant metric for deciding the accuracy of the system under test.

==> 5-discussion.tex <==
% !TEX root =  root.tex
\section{Discussion}\label{sec:discussion}
\lev{R2. discussion needed which model/approach to select for which purpose.}

\head{Factual Consistency}
Our framework showed a generally high performance on the task of evaluating factual consistency of conversational systems in the in-car domain, e.g., \carqa.

Some specific method and LLM combinations seem to work quite well for this task.
Taking all results into account, however, values from 20.3\% up to 92.2\% are reported.

The average was 72.5\%, the median at a way higher 82.5\%, meaning some method and LLM combinations scored particularly worse than the majority, reducing the average heavily.
GPT-3.5-turbo in combination with the Round-Table Conference and Chain-of-Thought only scored 20.8\% and 26.9\% respectively.
%These are not combinations that can be relied on.
The same happened with LLAMA 3 70B though, where we obtained a standard deviation of 25.9 points by changing the temperature.

% Upon inspection of our results, we noted the large difference in accuracy being due to easy and hard utterances. For example, GPT-4 with Input-Output prompting, which was originally designed to serve as a baseline, had an excellent performance of 91.3\% on easy tasks, but achieved only 75.7\% on hard tasks. This is a trend that was observed for almost all the methods tested.
% \andrea{we never introduce the difficulty of the task before, and this part could raise questions}

We conclude, that evaluations based on state-of-the art LLM models are promising to be used for factual consistency evaluations.

% and can, to an
% extent, be reliably used. We recommend relying on state-of-the-art LLMs for optimal performance. %, as other combinations perform significantly worse.

\head{Relevance}
\lev{Explan the best LLM model and technique.}For relevance, the accuracy of our framework was in general higher than for consistency.
With a median of 89.3\%, the majority of methods and LLM combinations achieved a  high agreement rate with human experts.

The highest score achieved was 93.2\% (GPT-3.5-turbo with IO and MPSC), though again the lowest
score (14.6\%, LLAMA 3 8B RT) drastically decreases the average score, which was 84.1\%.
Still, with a higher maximum score of 93.2\% than the results for factual consistency, lower standard deviation (14.8\%) and a higher median, using LLM for evaluations for relevance is recommendable. 
% The difference between the accuracy of easy and hard tasks exists here too, similar to the first metric, but has decreased for many methods due to the generally higher accuracy.

\head{Summary}
%At \company, prior to our work, the methods and LLMs were only examined for individual tasks, once for factual consistency with the source document and once for the relevance of the answer to the user utterance. 
%
The objective of our paper is to evaluate the factual correctness of the user utterance, which includes both metrics, an analysis is conducted to determine which method and LLM configuration performed best overall.
If we average the agreement rate with experts for both metrics, we find that the Round-Table Conference with GPT-4 and a temperature of 0.6 has outperformed all other combinations.
With an accuracy of 91.2\% for factual consistency and 92.2\% for relevance, this configuration achieved an average expert agreement rate of 91.7\%.
This is the highest overall accuracy achieved by any combination in the experiments performed, with the same configuration, but at different temperatures.

GPT-4 and Round-Table Conference with temperature 0.0 and 0.4 both achieved an average score of 91.2\%, the same as GPT-4 with Chain-of-Thought and a temperature of 0.6 and GPT-4 with standard Input-Output Prompting (temperature 0.0 and 0.2).
Of the top 15 results were obtained by GPT-4 \lev{Related to what??}, which confirms the state-of-the-art performance of this model~\cite{}.

As we are dealing with product-safety-relevant functions in the car and therefore have to make sure that
generated answers are as accurate possible, it all comes down to the little differences and to the last few percent that distinguishes the good results from the best.

For this reason, we recommend GPT-4 in combination with the Round-Table Conference approach, which has consistently delivered the best results.



==> figures/table_average_consistency.tex <==
\begin{table}[ht]
    \centering 
  \caption{Averaged accuracy scores for the different LLM and method combinations for factual consistency}
  \vspace{1em}
  \label{table:average_consistency}
\begin{tabular}{@{}llllll@{}}
\toprule
LLM        & IO   & CoT  & CoT-SC & MPSC & RT \\ \midrule
GPT-3.5-Turbo & \textbf{77.6} & 26.9 & 23.0   & 72.5 & 20.8        \\
GPT-4         & \textbf{91.2} & 89.0 & 89.3   & 84.9 & 90.2        \\
GPT-4o        & 78.8 & 64.4 & 63.3   & 79.6 & \textbf{85.6}        \\
LLAMA 3 8B    & 65.2 & 70.6 & 77.1   & 63.3 & \textbf{83.0}        \\
LLAMA 3 70B   & 83.7 & 84.7 & \textbf{84.9}   & 84.2 & 36.6        \\ \bottomrule
\end{tabular}
\end{table}

==> figures/table_average_relevance.tex <==
\begin{table}[ht]
    \centering 
  \caption{Averaged accuracy scores for the different LLM and method combinations for relevance}
  \vspace{1em}
  \label{table:average_relevance}
\begin{tabular}{@{}llllll@{}}
\toprule
LLM        & IO   & CoT  & CoT-SC & MPSC & RT \\ \midrule
GPT-3.5-Turbo & 90.2 & 89.0 & 89.8   & 91.2 & \textbf{92.7}        \\
GPT-4         & 90.2 & 91.5 & 91.7   & 79.1 & \textbf{92.2}        \\
GPT-4o        & 79.3 & 79.8 & 78.8   & 71.6 & \textbf{90.2}        \\
LLAMA 3 8B    & 85.1 & \textbf{86.6} & 85.1   & 66.7 & 15.0        \\
LLAMA 3 70B   & 91.2 & \textbf{91.5} & 91.2   & 83.0 & 91.2        \\ 
\bottomrule
\end{tabular}
\end{table}

==> figures/table_precision_recall_consistency.tex <==
\begin{table}[h]
    \centering 
  \caption{Precision and recall for selected LLM and method combinations for factual consistency}
  \vspace{1em}
  \label{table:consistency_precision_recall}
\begin{tabular}{llll}
\hline
LLM                     & Method & Precision & Recall \\ \hline
\multirow{5}{*}{GPT-4}  & RT     & 0.84      & 0.98   \\
                        & CoT    & 0.83      & 0.98   \\
                        & CoT-SC & 0.83      & 0.98   \\
                        & IO     & 0.86      & 0.97   \\
                        & MPSC   & 0.84      & 0.86   \\ \hline
\multirow{5}{*}{GPT-4o} & RT     & 0.81      & 0.96   \\
                        & CoT    & 0.91      & 0.56   \\
                        & CoT-SC & 0.91      & 0.56   \\
                        & IO     & 0.89      & 0.76   \\
                        & MPSC   & 0.88      & 0.76   \\ \hline
\end{tabular}
\end{table}


==> figures/table_precision_recall_relevance.tex <==
\begin{table}[ht]
    \centering 
  \caption{Precision and recall for selected LLM and method combinations for relevance}
  \vspace{1em}
  \label{table:relevance_precision_recall}
\begin{tabular}{llll}
\hline
LLM                     & Method & Precision & Recall \\ \hline
\multirow{5}{*}{GPT-4}  & RT     & 0.86      & 0.98   \\
                        & CoT    & 0.88      & 0.95   \\
                        & CoT-SC & 0.88      & 0.95   \\
                        & IO     & 0.88      & 0.93   \\
                        & MPSC   & 0.90      & 0.81   \\ \hline
\multirow{5}{*}{GPT-4o} & RT     & 0.86      & 0.96   \\
                        & CoT    & 0.95      & 0.71   \\
                        & CoT-SC & 0.95      & 0.71   \\
                        & IO     & 0.95      & 0.71   \\
                        & MPSC   & 0.96      & 0.62   \\ \hline
\end{tabular}
\end{table}


==> figures/table_temperature_settings_consistency.tex <==
\begin{table}[ht]
\centering
\caption{Agreement rate of LLM and method combinations with expert evaluation for factual consistency}
\vspace{1em}
\begin{tabular}{@{}llllll@{}}
                               &                                  & \multicolumn{4}{c}{Temperature}                   \\ \midrule
LLM                            & Method                           & 0.0        & 0.2        & 0.4        & 0.6        \\ \midrule
\multirow{5}{*}{GPT-3.5-turbo} & RT            & 21.3       & 20.3       & 20.3       & 21.3       \\
                               & CoT                 & 22.3       & 25.2       & 31.0       & 29.1       \\
                               & CoT-SC        & 22.3       & 22.3       & 24.2       & 23.3       \\
                               & IO                     & 82.5       & 81.5       & 76.6       & 69.9       \\
                               & MPSC & 72.8       & 74.7       & 72.8       & 69.9       \\ \midrule
\multirow{5}{*}{GPT-4}                          & RT            & 90.2 & 89.3 & 90.2 & 91.2 \\
                               & CoT                 & 89.3 & 88.3 & 88.3 & 90.2 \\
                               & CoT-SC        & 89.3 & 89.3 & 89.3 & 89.3 \\
                               & IO                     & 92.2 & 91.2 & 90.2 & 91.2 \\
                               & MPSC & 82.5 & 87.3 & 85.4 & 84.4 \\ \midrule
\multirow{5}{*}{GPT-4o}                         & RT            & 85.4 & 84.4 & 87.3 & 85.4 \\
                               & CoT                 & 65.0 & 65.0 & 64.0 & 64.0 \\
                               & CoT-SC        & 65.0 & 66.9 & 65.0 & 57.2 \\
                               & IO                     & 79.6 & 79.6 & 77.6 & 78.6 \\
                               & MPSC & 78.6 & 80.5 & 78.6 & 80.5 \\ \midrule
\multirow{5}{*}{LLAMA 3 70B}                    & RT            & 81.5 & 22.3 & 20.3 & 22.3 \\
                               & CoT                 & 84.4 & 84.4 & 84.4 & 85.4 \\
                               & CoT-SC        & 84.4 & 85.4 & 85.4 & 84.4 \\
                               & IO                     & 83.4 & 83.4 & 83.4 & 84.4 \\
                               & MPSC & 82.5 & 85.4 & 83.4 & 85.4 \\ \midrule
\multirow{5}{*}{LLAMA 3 8B}                     & RT            & 82.5 & 82.5 & 82.5 & 84.4 \\
                               & CoT                 & 52.4 & 79.6 & 76.6 & 73.7 \\
                               & CoT-SC        & 79.6 & 79.6 & 72.8  & 76.6 \\
                               & IO                     & 49.5 & 71.8 & 75.7 & 64.0 \\
                               & MPSC & 55.3 & 67.9 & 64.0 & 66.0 \\ \bottomrule
\end{tabular}
\label{table:temperature_consistency}
\end{table}

==> figures/table_temperature_settings_relevance.tex <==
\begin{table}[ht]
    \centering
    \caption{Agreement rate of LLM and method combinations with expert evaluation for relevance}
        \vspace{1em}
         \begin{tabular}{@{}llllll@{}}
                                       &                                  & \multicolumn{4}{c}{Temperature}                   \\ \midrule
        LLM                            & Method                           & 0.0        & 0.2        & 0.4        & 0.6        \\ \midrule
        \multirow{5}{*}{GPT-3.5-turbo} & RT            & 93.2 & 93.2 & 92.2 & 92.2 \\
                                       & CoT                 & 90.2 & 89.3 & 88.3 & 88.3 \\
                                       & CoT-SC        & 90.2 & 89.3 & 90.2 & 89.3 \\
                                       & IO                     & 90.2 & 89.3 & 92.2 & 89.3 \\
                                       & MPSC & 90.2 & 91.2 & 93.2 & 90.2 \\ \midrule
        \multirow{5}{*}{GPT-4}         & RT            & 92.2 & 92.2 & 92.2 & 92.2 \\
                                       & CoT                 & 92.2 & 91.2 & 90.2 & 92.2 \\
                                       & CoT-SC        & 92.2 & 92.2 & 91.2 & 91.2 \\
                                       & IO                     & 90.2 & 91.2 & 89.3 & 90.2 \\
                                       & MPSC & 82.5 & 77.6 & 77.6 & 78.6 \\ \midrule
        \multirow{5}{*}{GPT-4o}        & RT            & 91.2 & 89.3 & 90.2 & 90.2 \\
                                       & CoT                 & 78.6 & 80.5 & 79.6 & 80.5 \\
                                       & CoT-SC        & 78.6 & 79.6 & 77.6 & 79.6 \\
                                       & IO                     & 78.6 & 78.6 & 81.5 & 78.6 \\
                                       & MPSC & 70.8 & 71.8 & 71.8 & 71.8 \\ \midrule
        \multirow{5}{*}{LLAMA 3 70B}   & RT            & 91.2 & 91.2 & 91.2 & 91.2 \\
                                       & CoT                 & 91.2 & 91.2 & 91.2 & 92.2 \\
                                       & CoT-SC        & 90.2 & 91.2 & 91.2 & 92.2 \\
                                       & IO                     & 91.2 & 91.2 & 91.2 & 91.2 \\
                                       & MPSC & 82.5 & 82.5 & 82.5 & 84.4 \\ \midrule
        \multirow{5}{*}{LLAMA 3 8B}    & RT            & 14.5 & 15.5 & 14.5 & 15.5 \\
                                       & CoT                 & 85.4 & 85.4 & 89.3 & 86.4  \\
                                       & CoT-SC        & 85.4 & 85.4 & 86.4  & 83.4 \\
                                       & IO                     & 85.4 & 86.4  & 85.4 & 83.4 \\
                                       & MPSC & 66.9 & 66.0 & 72.8  & 61.1 \\ \bottomrule
        \end{tabular}
        \label{table:temperature_relevance}
        \end{table}
